Whisper: Fast Flooding for Low-Power Wireless Networks

This paper presents Whisper, a fast and reliable protocol to flood small amounts of data into a multi-hop network. Whisper makes use of synchronous transmissions, a technique first introduced by the Glossy flooding protocol. In contrast to Glossy, Whisper does not let the radio switch from receive to transmit mode between messages. Instead, it makes nodes continuously transmit identical copies of the message and eliminates the gaps between subsequent transmissions. To this end, Whisper embeds the message to be flooded into a signaling packet that is composed of multiple packlets -- where a packlet is a portion of the message payload that mimics the structure of an actual packet. A node must intercept only one of the packlets to detect that there is an ongoing transmission and that it should start forwarding the message. This allows Whisper to speed up the propagation of the flood, and thus, to reduce the overall radio-on time of the nodes. Our evaluation on the FlockLab testbed shows that Whisper achieves comparable reliability but 2x lower radio-on time than Glossy. We further show that by embedding Whisper in an existing data collection application, we can more than double the lifetime of the network.

==> sec/introduction_silvia.tex <==
%======================================================================================
\section{Introduction}
\label{sec:intro}
%======================================================================================

% \changed{
% % TODO
% % * Trade-off energy vs latency in dutcy-cycled networks
% % * Dissemination defined as flooding of small data into the network
% %OL: the text below is way too technical for the first section of the intro. We need to set the scene first. 
% Most communication protocols in low-power wireless networks are agnostic to the application on top of them.
% To be able to timely detect and handle communication requests, nodes must, nonetheless, regularly switch their radios on and check the channel for incoming transmissions. 
% While reducing the frequency and duration of this channel sampling procedure is mandatory to reduce energy consumption, frequent channel checks are needed to ensure a timely detection and handling of data traffic.
% Most wireless sensor network applications 
% %OL sentence broken
% }

\changed{Many application scenarios for low-power wireless networks require the reliable and fast exchange of small data values. Examples include the dissemination of parameters  -- e.g., the set-point of a valve -- in industrial control systems or smart buildings. 
% heating, ventilation and parameters may often need to be updated the set-points. 
% Examples include the dissemination of a 
% , changing the set-point for climate control or occupation driven HVAC in a smart building commonly relies on a single value. 
% Such events need to be relayed and acted upon by the building control system, which -- in low-power wireless networks -- is often multiple hops away from the event source.
% Similarly, industrial model-driven control supervises a control-loop and frequently updates the set-points. 
While such 
In these settings, the communication is either periodic or event-driven. 
Approaches like Glossy~\cite{Ferrari2011+Glossy} or LWB~\cite{Ferrari2012+LWB} can be used to  reliably and quickly share data periodically in a low-power wireless network. 
Crystal \cite{Istomin2016+Crystal,Istomin2018+Crystal2} and other approaches \cite{Sutton2015+Zippy, Istomin2018+Crystal2, Lim2017+Competition, Escobar2018+Competition, Trobinger2018+Competition, Ma2018+Competition, Nahas2018+Competition} extend Glossy to event-driven systems by periodically sampling the network for potential events.} 
%Nonetheless, both periodic and event-based applications commonly exchange small amounts of data.}

% For example, in Crystal \cite{Istomin2016+Crystal, } a control node frequently sends out a Glossy flood to which others nodes can reply in case of an event by sending their own flood.
% This sampling occurs in the order of hundreds of milliseconds to minutes, depending on application requirements \cite{Istomin2016+Crystal, Schuss2017+DepComp}.
% If multiple events have occurred in the network, their floods content to reach the initiating node. 
% Similar approaches based on frequent sampling are common in the EWSN dependability competitions \cite{Schuss2017+DepComp} since 2016 \cite{Lim2017+Competition,Escobar2018+Competition, Trobinger2018+Competition, Ma2018+Competition, Nahas2018+Competition}. 
% Depending on the exact application, events can be quite rare and as a result many of these floods do not trigger a reply, i.e., no actual data exchange.
% For example, in the temperature prediction scenario of Crystal less than 20\% of the sampling floods trigger a reply.
% As a result, this idle sampling of the network occurs a high communication overhead. 
% Moreover, when an event occurred they often only need to share an update of a single sensor value. 


\changed{In this paper, we present \name, a novel communication primitive that addresses the challenge of quickly and efficiently sharing small amounts of information in either periodic or event-based application scenarios.  
\name is a network primitive that builds upon synchronous transmissions and provides fast and energy-efficient communication in low-power wireless multi-hop networks. 
First, \name integrates the flood -- consisting of multiple replicated packets as in Glossy -- into a single packet transmission. 
This reduces the duration of a flood, eliminates gaps, i.e, the radio turnaround time, and thereby allows \name to reduce radio-on time and energy consumption.
    Second, its compact flooding format and the lack of gaps between packets enable \name to introduce energy-efficient sampling strategies, i.e, the ability to sample the channel for a packet and not, as done in Glossy, LWB, Crystal and most others protocols to rely on idle listening of the radio.}
    
\changed{\name can be used as \enquote{standalone} dissemination protocol for small data and as service for other protocols, e.g., as an efficient wake-up primitive to reduce the protocols idle listening overhead. 
    The latter is the case in the event-based transmission of large data packets. 
    In such scenarios, the nodes listen to potential packets for a predefined interval before turning the radio off.
    Using \glossy-like protocols, the length of this interval depends on the packet size, the number of hops in the network, and the number of packet repetitions~$N_{tx}$. 
    For example, it would take \glossy almost 67~ms to disseminate a 127~byte packet in a 6-hop network with $N_{tx} = 3$. 
    Thus, all nodes must keep the radio turned on for the this amount of time even when no packet is disseminated.
    Using \name, the nodes keep their radio on for at most a \name slot, which is less than 3~ms in a 6-hop network. 
    Only if they have received a packet during the Whisper slot, they await the actual data packet afterwards. 
    Otherwise, they keep their radio turned off. 
    Thus, using \name, nodes only communicate when they have an event to share. 
%     In sum, in case of no data traffic, the nodes are awake using \name for only 3 ms~instead of 67~ms.
}

%\name is a new network-wide primitive for  \changed{periodic as well as event-based} communication. 
%It builds on synchronous transmissions as introduced by Glossy and provides fast and energy-efficient communication in multi-hop low-power wireless networks.
%In \name, nodes only initiate communication during a communication round when they have an event to share (next to infrequently scheduled rounds for time synchronization) and, as a result, no frequent communication floods as in Crystal are required. 
%Moreover, nodes sample the medium during the communication time, and are not, as in other approaches, constantly active during the potential duration of the network flood.
%For example, in Crystal, a network flood commonly takes 5~ms to 8~ms for networks of 30 ~nodes (Flocklab testbed) and 90 ~nodes, respectively (Indriya testbed). 
%%In contrast, in \name nodes -- in best case -- only sample once for less than a half a millisecond per communication round.
%In contrast, with \name nodes sample typically less than 3~ms per communication round.
%Finally, \name makes network-floods significantly shorter by integrating the flood into a single packet transmission.
%This (a) reduces the duration of a flood and thereby allows \name to reduce radio-on time and reduce energy consumption and (b) enables robust sampling as in \name there is no gap between two packets. 

In summary, \name is designed around three cornerstones:
\begin{itemize}	
\item \name compacts the network flood into a single packet without \enquote{gaps} to reduce latency and radio-on time and enable efficient sampling.
\item \name employs strategies \changed{for} sampling so that nodes can determine at high energy efficiency whether there is data exchange during a round or not.
\item \changed{\name exploits synchronous transmissions for fast and reliable flooding.}
%\item \name limits communication to rounds where there is actual data to exchange (plus infrequent rounds for clock synchronization). 
%\item \name employs strategies \changed{for} sampling so that nodes can determine at high energy efficiency whether there is data exchange during a round or not.
%\item When there is data to exchange, \name compacts the network flood into a single packet without \enquote{gaps} to reduce latency and radio-on time and enable efficient sampling. 
\end{itemize}
%Each of these three design elements improves the performance of synchronous transmissions in the context of \changed{event-based} communication when, for example, added to Glossy. 
%However, we show in our design analysis and evaluation that the careful design and combination of these three elements amplifies their benefits and is the root over our manifold performance improvements.

\changed{We show the efficiency of \name as primitive for fast and efficiency network-wide signaling by evaluating it on the publicly available FlockLab testbed.}
%We show the efficiency of \name as primitive for fast and efficiency network-wide signaling by evaluating it on two publicly available testbeds, Flocklab and Indriya.
For example, in \name nodes can determine whether a flood is ongoing within less than 3~milliseconds \changed{in a 6-hop network} whereas in Crystal and in several solutions of the EWSN dependability competitions, nodes are awake for the duration of the network flood, which on Flocklab, for example, commonly takes 5~milliseconds. 
\changed{We further show that \name has a up to 50\% higher network lifetime than Glossy and it can increase the network lifetime of Crystal by a factor of 2.3 when used as wake-up service within Crystal.}
%\OL{
%
%In addition, ...
%%TODO OL some more results here
%
%%TODO OL: once the above text is stable and design + eval become stable, we shall summarize here
%Once the abobe text is I need three numbers to be discussed in our call on Friday:
%* sampling duration of FastWake and on-time of Crystal during idle sampling
%* duration of flood in Fastawke and compared to Crystal
%* overall improvements over Crystal: of idle duty cycle
%}
% %\MB{Fix later from here.}
% %Our results show the ability of \name to provide for a better energy-latency trade-off than its closest competitors.
% We observe that \name wakes-up an entire network of 27 nodes and 4 hops by having the nodes turned on their radio for only 2.6~milliseconds.
% Integrated as wake-up primitive can \name reduce the overall energy consumption of a protocol by more than 21\% as we show on the example of Crystal~\cite{Istomin2016+Crystal} and LaneFlood~\cite{Brachmann16+LaneFlood}, two recently proposed protocols with on-demand traffic patterns.
% We show that \name improves efficiency by factor X when compared to Crystal.
% Moreover, we show the flexibility of \name by integrating it into LaneFlood 
% %OL: todo cite
% , a extension to Glossy that limits directs network floods to the path between two nodes. 


%If regular wake-up intervals of 30 seconds are scheduled, \name has a idle duty cycle of 0.06\% (including synchronization).
%For wake-up intervals of 30 seconds, this comes at a duty cycles of just 0.06\% (including synchronization).
%In comparable settings, Crystal~\cite{Istomin2016+Crystal}, a recently proposed approach for data collection achieves a duty cycle of 0.1\%.

%Section \ref{sec:overview} introduces the basic idea of \name.
%Next, Section \ref{sec:details} discusses the design choices of \name in detail. 
%We evaluate \name and compare its performance to the state of the art in Section \ref{sec:eval}.
%Section \ref{sec:related_work} presents the related work and discusses key differences of \name. 
%We conclude in Section \ref{sec:conclusion}.

The remainder of this article is structured as follows.
We present a high-level overview of \name in Section \ref{sec:overview} and discuss relevant details of its design in Section \ref{sec:details}.
Using our implementation for TelosB nodes in Contiki, we compare \name in various dissemination scenarios with \glossy in  Sec.~\ref{sec:eval} and use \name as wake-up primitive in Crystal in Sec.~\ref{sec:eval_crystal}.
%We then detail on implementation details of \name in \ref{} and present the evaluation of \name in Section \ref{}.
A discussion of related work follows in Sec.~\ref{sec:related_work} and Sec.~\ref{sec:conclusion} concludes the paper.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% VERY OLD STUFF BELOW THIS POINT %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\todo{fix refs to Sections.}


%Koala achieves very low average network wake-up time of 29 seconds


%to be available with very high probability whenever they are necessary for communication
%
%if nodes do not wake up frequently, they might not be available for communication when needed.
%


% A common technique to save energy in wireless networks consists in letting nodes keep their radios off for possibly long periods of time.
% In this \emph{sleep mode}, nodes cannot communicate and their radio circuitry consumes little or no power.
% To receive and forward incoming transmissions or to send own data, nodes need to wake-up from this sleep mode.
% For nodes to be able to communicate with each other, though, they must be awake in the same temporal interval.
% %A common problem in low-power networks is thus that of rendezvousing sleeping nodes, i.e., to ensure that they wake up together.
% %This is especially the case for event-based communication, where the communication intervals are not known beforehand and thereby the system cannot synchronize to a schedule.
% While they enable this \emph{rendezvous} between nodes, wake-up protocols must cope with a fundamental trade-off between energy consumption and latency.
% %Wake-up protocols must thus enable this \emph{rendezvous} between nodes and need to cope with a fundamental trade-off between energy consumption and latency.
% The longer nodes keep their radios off, the more energy they can save.
% On the other side, the more often nodes resume from sleep mode to listen to potentially incoming communications, the shorter it takes for a communication attempt to be served.
% %This is because the more often nodes resume from sleep mode to listen to potentially incoming communications, the lesser the risk of losing a ``wake-up'' call.

% Waking up the entire network is necessary whenever collaboration of all nodes is needed.
% This is for example the case when information needs to be distributed quickly into the network and sleeping nodes may delay the communication.
% Furthermore, some communication protocols -- in particular those based on synchronous transmissions~\cite{Ferrari11+Glossy, Ferrari2012+LWB, Landsiedel2013+Chaos, Istomin2016+Crystal, Brachmann16+LaneFlood} -- require all nodes to be awake to operate.

% Several wake-up protocols already exist, including Koala~\cite{Musaloiu08+Koala}, Zippy~\cite{Sutton2015+Zippy}, ALBA-WUR~\cite{Spenza2015+ALBA-WUR}, STEM~\cite{Schurgers2002+STEM}, and others~\cite{Liu2016+Network-Wide-Wakeup, Miller2005+Wakeup+Radio, Dhanaraj2005+LEEM, Yang2004+PTW}.
% A drawback of existing network-wide wake-up protocols is that they usually optimize for energy savings and thus induce high latency in the communication.
% For instance, Koala needs several minutes to wake up a network of few tens of nodes~\cite{Musaloiu08+Koala}.
% Other approaches offer a better trade-off between energy and latency, but rely on dedicated hardware like, e.g., wake-up radios~\cite{Sutton2015+Zippy, Spenza2015+ALBA-WUR, Liu2016+Network-Wide-Wakeup, Magno2016+WUR}.
% %Wake-up radio have two key limitations:
% %(1)~their additional dedicated hardware increases the complexity and price of a networked node, and
% %(2)~the limited range of wake-up radios.
% %Most wake-up radios have a passive design, i.e., they do not employ active components such signal amplifiers, to ensure energy efficiency~\cite{Sutton2015+Zippy, x, y, z}.

% In this paper, we present \name, a communication primitive that provides a fast and energy-efficient wake-up for multi-hop wireless networks.
% Any node in the network can initiate the wake-up, thus \name can effectively support on-demand traffic patterns.
% Furthermore, network protocols can utilize \name as a basic service to wake-up the network before they start their own operation.
% By decoupling the network wake-up functionality from communication, \name eases the design of network protocols.
% %\name bases on synchronous transmissions and does not require additional hardware such as wake-up radios.
% %This primitive is particularly useful when the expected traffic is sporadic and event-based.
% %In these scenarios, \name ensures that a network will wake-up quickly whenever a node needs to communicate.
% %\name ensures that all nodes within a network of several hops can be awaken within few milliseconds.

% \name relies on three main cornerstones: %ACHTUNG: lwb ALSO SAYS "WE RELY ON THREE CORNERSTONES"
% \begin{itemize}
	
% \item It exploits synchronous transmissions to quickly flood a ``wake-up call'' through the network.
% This ensures low energy consumption since nodes only need to be awake for few milliseconds to verify whether there is an incoming wake-up call or not.
% \name allows any node to wake-up the network and can thus serve on-demand traffic patterns.

% \item It minimizes the risk of a node missing the wake-up call by composing the wake-up message as a series of \emph{\packlets}.
% A \packlet is a portion of the data payload that mimics the structure of an actual packet (preamble, start-of-frame delimiter, etc.).
% This enables nodes to `'lock-in'' into the wake-up message irrespectively of when they starts receiving it.

% \item It provides strategies to reduce the idle listing time of potentially incoming \packlets and therefore, lowers the overall radio duty cycle of the nodes.
% %\Packlets are sent back-to-back without gaps between transmissions, which allows for the design of novel sampling strategies.
% %\MB{strategies depend on traffic pattern and so on}
% %\MB{Text is now in abstract}

% \end{itemize}

% %\MB{Fix later from here.}
% We evaluate the performance of \name on two publicly available testbeds, Flocklab and Indriya.
% %Our results show the ability of \name to provide for a better energy-latency trade-off than its closest competitors.
% We observe that \name wakes-up an entire network of 27 nodes and 4 hops by having the nodes turned on their radio for only 2.6~milliseconds.
% Integrated as wake-up primitive can \name reduce the overall energy consumption of a protocol by more than 21\% as we show on the example of Crystal~\cite{Istomin2016+Crystal} and LaneFlood~\cite{Brachmann16+LaneFlood}, two recently proposed protocols with on-demand traffic patterns.
% %If regular wake-up intervals of 30 seconds are scheduled, \name has a idle duty cycle of 0.06\% (including synchronization).
% %For wake-up intervals of 30 seconds, this comes at a duty cycles of just 0.06\% (including synchronization).
% %In comparable settings, Crystal~\cite{Istomin2016+Crystal}, a recently proposed approach for data collection achieves a duty cycle of 0.1\%.

% %The remainder of this paper is structured as follows.
% %We present a high-level overview of \name in Section \ref{sec:overview} and discuss relevant details of its design in Section \ref{sec:overview}.
% %We then describe \name's implementation for the Contiki operating system in Section \ref{} and report about the evaluation of our approach in Section \ref{}.
% %A discussion of our as well as relate work follows in Section \ref{} and Section \ref{}.
% %Finally, Section \ref{} concludes the paper.
% %\todo{fix refs to Sections.}



% %Koala achieves very low average network wake-up time of 29 seconds


% %to be available with very high probability whenever they are necessary for communication
% %
% %if nodes do not wake up frequently, they might not be available for communication when needed.
% %
%
%
%Nodes must wake-up with very high probability whenever they are necessary for communication.
%
%
%The risk of a nodes missing a ``wake-up call'',
%
%need to overcome consist in needs to be overcome is tha
%
%Most of the approaches in the existing literature achieve low energy consumption by scarifying latency.
%In


%Any-to-any wake-up. For this reason nodes need to be awake during the whole window

%We need to wake up all nodes with very high probability; risk of a node missing the wake-up must be very low;
%At the same time, the wake up must be quick;
%And we should not use too much energy;






%Thereby, we also build zupon techniques that are
%
%present a novel protocol, called \name, that wakes-up an entire network in a fast and energy-efficient manner.
%
%
%
%provides a simple primitive to quickly wake-up an entire
%
%The more often the nodes wake-up, the more probable it is they will not miss a communication attempt.
%There is thus an intrinsic trade-off between the frequency and duration of wake-ups -- and the related energy consumption -- and the resulting latency and even reliability of the communication.



%\subsection{Silvia's notes}
%
%Other approaches instead focus on ensuring that the entire network is awake before data transmission starts.
%
%Thsi is in pareticular needed when all nodes in the network are required to collaborate in data transmissions.
%This is for exmaple the case in collection and dissemination.
%In particular this also occurs when protocols based on synchronous transmissions are used.
%These appraoches need the entire network -- or at least a large part  thereof -- to be awake to work properly.
%
%In general, there exist a trade-off between how often nodes wake up.
%
%
%A typical approach consists in making nearby nodes wake-up at the same time instant.
%This requires the nodes to be synchronized and agree on the wake-up time.
%This technique is used in many well-know approaches [ADD REFERENCES].
%While some techniques focus on ensuring 1-hop neighboring nodes can wake-up at the same time, other approaches aim at waking up the entire network before data transmission starts.
%The latter include Koala, XY, and ZW.


%\subsection{Martina's draft under this point}
%
%\DEBUG{Motivation.}
%
%On-demand traffic is an essential application requirement in wireless sensor networks (WSNs). In the last decades research focused on .... protocols like the Constrained Application Protocol (CoAP) or data prediction. The overall goal is to reduce the message overhead in the resouce-constrained network so that nodes are in sleep mode most of the time to preserve energy. However, there is a trade-off between nodes that have there radio turned off most of the time and the overall end-to-end latency of a packet in case of an event.
%In this paper we introduce \name, a novel protocol primitive that wakes up nodes in a  network with over X hops in less than XX~ms. When the nodes are awake, any protocol can take over to perform the message exchange in a quick mannner as all nodes are awake.
%
%Application scenarios range from request-response applications as it is supported with e.g. the Constrained Application Protocol (CoAP), to data prediction and data fusion applications, where only pre-processed, relevant data is sent to a sink node \cite{Istomin2016+Crystal, Gungor2009+Survey}.
%
%\MB{Whats an event? Describe on examble.}
%
%%event-triggered communication / on demand traffic trade-off latency and duty cycle
%
%%periodic traffic good / time synchronisation goes hand in hand
%
%%nodes can wakeup in a period of time but dont know exactly when to wakeup
%
%%synchronisation; applications often require a common sense of time e.g. for timestamping the reported data.
%
%%trade-off between duty cycle and  latency in event-based communication schemes.
%
%
%\DEBUG{Challenge.}
%The key challenge is to exchange on-demand traffic with low latency and low duty-cycle. An event happens only on rare occasions, that means most of the times the nodes are in sleep mode to save energy. However, in sleep mode, the nodes cannot send or receive events. %TODO: Make it more concrete with an example. why does low-power probing/listing not help in our example? Whats the drawback of glossy? Whats the drawback of crystal. What about special hardware like zippy or backscatter?
%
%
%%After long phases of no communication, an event triggers active communication between nodes. When an event happens, usually several nodes need to be involved in the communication. That is because either several nodes have sensed the same event and want to report their data to e.g. a controller or, a pair of nodes have to exchange several data packets (e.g. CoAP) over multiple hops.
%
%%\begin{itemize}
%%	\item \emph{Trade-off between duty cycle and  latency in event-based communication schemes}.
%%	
%%	\item Glossy enables native node \emph{synchronization with no cost through periodic packets}. In case only a fixed number of nodes triggers communication, the other nodes can sample the channel at a fixed point in time as they know with Glossy when to expect a packet. When every node in the network can send packets, the nodes have to sample within an interval, which length depends on the network diameter.
%%\end{itemize}
%
%\DEBUG{Approach.}
%The nodes wakeup, sample and if no message, nodes go to sleep. If message, the receiving nodes join in sending the exact same message so nodes that are several hops away from the initial sender of the message, have also a chance to receive it.
%
%\DEBUG{Contributions.}
%\begin{itemize}
%	\item A primitive that wakes up reliably XX\% of the nodes in a multi-hop network within a few milliseconds. After all nodes have woken up one or multiple nodes  that have event-data to distribute can exchange data.
%	\item We provide a method to compensate clock drift.
%	\item We demonstrate in testbed experiments the robustness of our design and show that our protocol achieves improvements compared to state of the art protocols
%	\item
%\end{itemize}
%
%\DEBUG{Outline.} 
